Collaborative Vision-Text Representation Optimizing for Open-Vocabulary Segmentation

Pre-trained vision-language models, e.g. CLIP, have been increasingly used to address the challenging Open-Vocabulary Segmentation (OVS) task, benefiting from their well-aligned vision-text embedding space. Typical solutions involve either freezing CLIP during training to unilaterally maintain its zero-shot capability, or fine-tuning CLIP vision encoder to achieve perceptual sensitivity to local regions. However, few of them incorporate vision-text collaborative optimization. Based on this, we propose the Content-Dependent Transfer to adaptively enhance each text embedding by interacting with the input image, which presents a parameter-efficient way to optimize the text representation. Besides, we additionally introduce a Representation Compensation strategy, reviewing the original CLIP-V representation as compensation to maintain the zero-shot capability of CLIP. In this way, the vision and text representation of CLIP are optimized collaboratively, enhancing the alignment of the vision-text feature space. To the best of our knowledge, we are the first to establish the collaborative vision-text optimizing mechanism within the OVS field. Extensive experiments demonstrate our method achieves superior performance on popular OVS benchmarks. In open-vocabulary semantic segmentation, our method outperforms the previous state-of-the-art approaches by +0.5, +2.3, +3.4, +0.4 and +1.1 mIoU, respectively on A-847, A-150, PC-459, PC-59 and PAS-20. Furthermore, in a panoptic setting on ADE20K, we achieve the performance of 27.1 PQ, 73.5 SQ, and 32.9 RQ. Code will be available at https://github.com/jiaosiyu1999/MAFT-Plus.git .

==> figs/tex/4-text.tex <==
% \begin{figure}[t]
% % \vspace{-10mm}
% \begin{center}
%    \includegraphics[width=0.99\linewidth]{figs/pdf/text.pdf}
% \end{center}
% \vspace{-3mm}
%    \caption{
%     Comparisons between CLIP-Text tuning strategies. 
%    }
% \label{fig:text}
% % \vspace{-5mm}
% \end{figure}


\noindent\makeatletter\def\@captype{figure}\makeatother
\begin{minipage}{1.0\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{figs/pdf/text.pdf}
       \caption{
        Comparisons between CLIP-Text tuning strategies. 
       }
    \label{fig:text}
    \end{minipage} \\
    
\noindent\makeatletter\def\@captype{table}\makeatother
    \begin{minipage}{1.0\textwidth}
    \centering
    \footnotesize
      % \vspace{-10pt}
  \caption{\textbf{Ablation of diverse designs of CLIP-Text optimization.} We remove the Representation Compensation strategy and freeze CLIP-V for analysis. Note that fine-tuning CLIP-T requires excessive GPU memory, and thus it is infeasible (denoted as $\mathrm{N/A}$) for the setting in the 2$^{nd}$ row.
}
   % \vspace{-10pt}
  % \begin{threeparttable}  
  % \resizebox{1.0\textwidth}{
    \renewcommand\arraystretch{1.05} % 1.95
    % \begin{tabular}{l|ccccc}
    \begin{tabular}{l|lllll}
      % \toprule
      \Xhline{0.7pt}

      & \textbf{A-847} & \textbf{A-150} & \textbf{PC-459} & \textbf{PC-59} & \textbf{PAS-20}\\ 
      \hline
      frozen CLIP (baseline)&  ~~11.2 & ~~26.6 &  ~~12.7  &  ~~42.4 & ~~89.5 \\     
      + fine-tune CLIP-T&  ~~$\mathrm{N/A}$ & ~~$\mathrm{N/A}$ &  ~~$\mathrm{N/A}$  &  ~~$\mathrm{N/A}$ & ~~$\mathrm{N/A}$ \\     
      + MLP &  ~~4.1  & ~~20.2 &  ~~11.2  &  ~~51.4 & ~~89.4 \\     
      + GPT-Descriptions &  ~~11.9  & ~~28.2 &  ~~13.3  &  ~~42.6 & ~~90.6 \\     
      + Llama-Descriptions &  ~~9.6  & ~~26.1 &  ~~11.5  &  ~~40.8 & ~~90.9 \\ 
      \rowcolor{gray!10}\multicolumn{1}{c|}{+ Content-Dependent Transfer}
       &  ~~\textcolor{red}{13.3} & ~~\textcolor{red}{32.4} &  ~~\textcolor{red}{17.2} &  ~~\textcolor{red}{55.2} & ~~\textcolor{red}{94.7} \\     
      \Xhline{0.7pt}
      \end{tabular}
      % }
      \label{tab:cd}
    % \vspace{5mm}
    \end{minipage}

==> tables/name.tex <==
\begin{table}[t]
  \centering
  \footnotesize
  \caption{Open-vocabulary \textit{semantic} segmentation performance. mIoU is used to evaluate the performance. * denotes additional ensemble operation \cite{fcclip} used during testing. }
  % \resizebox{1.0\textwidth}{!}{
    \renewcommand\arraystretch{1.05} % 1.95
    % \begin{tabular}{l|ccccc}
    \begin{tabular}{l|lllll}
      % \toprule
      \Xhline{0.7pt}

      & \textbf{A-847} & \textbf{A-150} & \textbf{PC-459} & \textbf{PC-59} & \textbf{PAS-20}\\ 
      \hline
      OVSeg \pub{CVPR23}\cite{ovseg} & 7.1 & 24.8 & 11.0 & 53.3 & 92.6\\
      OpenSeg \pub{ECCV22}\cite{ghiasi2022scaling} &  8.8 & 28.6 & 12.2  &  48.2 & 72.2\\ 
      SAN \pub{CVPR23}\cite{san} &  12.4 & 32.1 &  15.7  &  57.7 & 94.6 \\     
      ODISE \pub{CVPR23}\cite{odise} &  11.1 & 29.9 &  14.5  &  57.3 &  - \\     
      FC-CLIP \pub{NeurIPS23}\cite{fcclip} &  11.2 & 26.6 &  12.7  &  42.4 & 89.5 \\   
      FC-CLIP* \pub{NeurIPS23}\cite{fcclip} &  14.8 & 34.0 &  18.2  &  58.4 & 95.4 \\   
      MAFT \pub{NeurIPS23}\cite{maft} &  12.7 & 33.0 &  16.2  &  59.0 & 92.1 \\     
      \cdashline{1-6}[0.8pt/2pt]
      % MAFT+ (ours) & \textbf{15.3} & \textbf{36.1} & \textbf{21.6} & \textbf{59.4} & \textbf{96.5} \\
      MAFT+ (ours) & 15.3 $_{\textcolor{red}{+0.5}}$ & 36.3 $_{\textcolor{red}{+2.3}}$ & 21.6 $_{\textcolor{red}{+3.4}}$ & 59.4 $_{\textcolor{red}{+0.4}}$ & 96.5 $_{\textcolor{red}{+1.1}}$ \\
      \Xhline{0.7pt}
      % \bottomrule
      \end{tabular}
      % }
      % \end{threeparttable}
      \label{tab:ovs}
  \vspace{-2mm}
  \end{table}  

==> tables/rc-loss.tex <==
\begin{table}
  \centering
  \footnotesize
  % \vspace{-10pt}
  \caption{Ablation of the loss functions in Representation Compensation. The Content-Dependent Transfer is removed.
}
    \renewcommand\arraystretch{1.05} % 1.95
    % \begin{tabular}{l|ccccc}
    \begin{tabular}{c|lllll}
      % \toprule
      \Xhline{0.7pt}

      & \textbf{A-847} & \textbf{A-150} & \textbf{PC-459} & \textbf{PC-59} & \textbf{PAS-20}\\ 
      \hline
      $\mathrm{L_1}$ &  ~~ & ~~ &  ~~  &  ~~ & ~~ \\     
      \rowcolor{gray!10}\multicolumn{1}{c|}{$\mathrm{SmoothL1}$}&  ~~ & ~~ &  ~~  &  ~~ & ~~ \\     
      $\mathrm{L_2}$&  ~~ & ~~ &  ~~  &  ~~ & ~~ \\     
      $\mathrm{KL}$ &  ~~ & ~~ &  ~~  &  ~~ & ~~ \\     

      \Xhline{0.7pt}
      % \bottomrule
      \end{tabular}
      % }
      % \end{threeparttable}
      \label{tab:RC-loss}
  \vspace{-2mm}
  \end{table}  


==> tables/rc-unit.tex <==

\begin{table}
  \centering
  \footnotesize
  % \vspace{-10pt}
  \caption{Ablation of the frozen units in CLIP-Vision. The Content-Dependent Transfer is removed.
}
    \renewcommand\arraystretch{1.05} % 1.95
    % \begin{tabular}{l|ccccc}
    \begin{tabular}{l|lllll}
      % \toprule
      \Xhline{0.7pt}

      & \textbf{A-847} & \textbf{A-150} & \textbf{PC-459} & \textbf{PC-59} & \textbf{PAS-20}\\ 
      \hline
      None &  ~~14.6 & ~~34.8 &  ~~18.2  &  ~~57.1 & ~~95.3 \\     
      Freeze \{S0\}&  ~~ & ~~ &  ~~  &  ~~ & ~~ \\     
      Freeze \{S0, S1\}&  ~~ & ~~ &  ~~  &  ~~ & ~~ \\     
      Freeze \{S0, S1, S2\}&  ~~ & ~~ &  ~~  &  ~~ & ~~ \\     

      \Xhline{0.7pt}
      % \bottomrule
      \end{tabular}
      % }
      % \end{threeparttable}
      \label{tab:RC-unit}
  \vspace{-2mm}
  \end{table}  





==> tables/rebuttal-all.tex <==

\begin{table}[!t]
% \caption{xxxxxxx.}
\label{tab:reb}
    %%%%%%%%%%%%%%%%%%%%%% tab 1 %%%%%%%%%%%%%%%%%%%%%
    \hspace*{-1.5cm}
  \begin{subtable}{0.25\textwidth}
    \centering
    \setlength{\belowcaptionskip}{-0.5cm}
    \setlength{\tabcolsep}{1pt}
    \scriptsize

    \begin{tabular}{l|ccccc}
        \toprule[1pt]
         & A-847 & A-150 & PC-459 & PC-59
        \tabularnewline
        \midrule[1pt]
        MAFT-ViTL & 12.7 & 33.0 & 16.2 & 59.0\\
        MAFT-ConvnextL &13.1 & 34.4 & 17.0 & 57.5\\
        MAFT+ (ours) &15.1 & 36.1 & 21.6 & 59.4\\
        \bottomrule[1pt]
    \end{tabular}

    \hspace*{0.75cm}

    \caption{Comparison with different variations of MAFT.}
    \label{reb-maft}
  \end{subtable}%
    %%%%%%%%%%%%%%%%%%%%%% tab 2 %%%%%%%%%%%%%%%%%%%%%
    \hspace*{0.75cm}
  \begin{subtable}{0.25\textwidth}
    \centering
    \setlength{\belowcaptionskip}{-0.5cm}
    \setlength{\tabcolsep}{1pt}
    \scriptsize

    \begin{tabular}{l|ccccc}
        \toprule[1pt]
         & A-847 & A-150 & PC-459 & PC-59
        \tabularnewline
        \midrule[1pt]
        \textit{w.o.} $\mathcal{L}_{dis}$ [\textcolor{eccvblue}{17}] \& RC & 12.6 & 33.8 & 16.4 & 55.4 \\
        + $\mathcal{L}_{dis}$ [\textcolor{eccvblue}{17}] &12.4  & 33.9 & 16.7 & 55.8 \\
        + RC (ours) &14.6 & 34.8 & 18.2 & 57.1 \\
        \bottomrule[1pt]
    \end{tabular}

    \caption{Comparison between $\mathcal{L}_{dis}$ [\textcolor{eccvblue}{17}] and RC. CDT is removed}
    \label{reb-ldis}
  \end{subtable}

    \hspace*{0.75cm}

    %%%%%%%%%%%%%%%%%%%%%% tab 3 %%%%%%%%%%%%%%%%%%%%%
    \hspace*{-1cm}
  \begin{subtable}{0.25\textwidth}
    \centering
    \setlength{\belowcaptionskip}{-0.5cm}
    \setlength{\tabcolsep}{1pt}
    \renewcommand\arraystretch{0.8} % 1.95
    \scriptsize

    \begin{tabular}{l|ccccc}
        \toprule[1pt]
         & ~A-847 & ~A-150 & ~PC-459 & ~PC-59
        \tabularnewline
        \midrule[1pt]
        ~SAN & 12.6 & 33.8 & 16.4 & 55.4 \\
        ~SAN\dag  &12.4  & 33.9 & 16.7 & 55.8 \\
        ~FreeSeg & 7.1 & 17.9 & 6.4 & 34.4 \\
        ~FreeSeg\dag ~ &-  & - & - & - \\
        \bottomrule[1pt]
    \end{tabular}

    \caption{Adapting to other frameworks. \dag denote using our optimizing strategy.}
    \label{reb-san}
  \end{subtable}
    %%%%%%%%%%%%%%%%%%%%%% tab 4 %%%%%%%%%%%%%%%%%%%%%
    \hspace*{0.2cm}
  \begin{subtable}{0.25\textwidth}
    \centering
    \setlength{\belowcaptionskip}{-0.5cm}
    \setlength{\tabcolsep}{1pt}
    \renewcommand\arraystretch{0.8} % 1.95
    \scriptsize

    \begin{tabular}{l|cc}
        \toprule[1pt]
         & ~~COCO~~ & ~~COCO+LVIS~~
        \tabularnewline
        \midrule[1pt]
        A-847~ & 6.1 & 25.7 \\
        A-150 &26.7 & 46.7 \\
        PC-459~ & 16.1 & 57.0 \\
        PC-59  &59.3  & 66.1 \\
        \bottomrule[1pt]
    \end{tabular}

    \caption{Proportion of the train-test overlapping classes.}
    \label{reb-overlap}
  \end{subtable}
\end{table}


==> tables/rebuttal-ldis.tex <==
\begin{table}[h]
% \vspace{-4mm}
\centering
\setlength{\belowcaptionskip}{-0.5cm}
\setlength{\tabcolsep}{3pt}
\scriptsize
% \footnotesize
    \begin{tabular}{l|ccccc}
        \toprule[1pt]
         & A-847 & A-150 & PC-459 & PC-59 & PAS-20 
        \tabularnewline
        \midrule[1pt]
        \textit{w.o.} $\mathcal{L}_{dis}$ \& RC & 12.6 & 33.8 & 16.4 & 55.4 & 94.1 \\
        + $\mathcal{L}_{dis}$  &12.4  & 33.9 & 16.7 & 55.8 & 93.2 \\
        + RC (ours) &14.6 & 34.8 & 18.2 & 57.1 & 95.3 \\
        \bottomrule[1pt]
    \end{tabular}
% \vspace{-2mm}
\caption{Comparison between $\mathcal{L}_{dis}$ and RC. CDT is removed.
% We first retrain the network \textit{w.o.} $\mathcal{L}_{dis}$ and RC, and then add each loss gradually.
}
\label{reb-ldis}
\end{table}

==> tables/rebuttal-maft.tex <==
\begin{table}[h]
% \vspace{-4mm}
\centering
\setlength{\belowcaptionskip}{-0.5cm}
\setlength{\tabcolsep}{3pt}
\scriptsize
% \footnotesize
    \begin{tabular}{l|ccccc}
        \toprule[1pt]
         & A-847 & A-150 & PC-459 & PC-59 & PAS-20 
        \tabularnewline
        \midrule[1pt]
        MAFT-ViTL & 12.7 & 33.0 & 16.2 & 59.0 & 92.1\\
        MAFT-ConvnextL &13.1 & 34.4 & 17.0 & 57.5 &94.0\\
        MAFT+ (ours) &15.1 & 36.1 & 21.6 & 59.4 &96.5 \\
        \bottomrule[1pt]
    \end{tabular}
% \vspace{-2mm}
\caption{Comparison with different variations of MAFT.}
\label{reb-maft}
\end{table}

==> tables/rebuttal-overlap.tex <==
\begin{table}[h]
% \vspace{-4mm}
\centering
\setlength{\belowcaptionskip}{-0.5cm}
\setlength{\tabcolsep}{3pt}
\scriptsize
% \footnotesize
    \begin{tabular}{l|ccccc}
        \toprule[1pt]
         & A-847 & A-150 & PC-459 & PC-59 & PAS-20 
        \tabularnewline
        \midrule[1pt]
        COCO & 6.1\% & 26.7\% & 16.1\% & 59.3\% & 100\% \\
        COCO+LVIS &25.7\% & 46.7\% & 57.0\% & 66.1\% &100\% \\
        \bottomrule[1pt]
    \end{tabular}
% \vspace{-2mm}
    \caption{Proportion of the train-test overlapping categories.}
\label{reb-overlap}
\end{table}

==> tables/rebuttal-params.tex <==
\begin{table}[h]
% \vspace{-4mm}
\centering
\setlength{\belowcaptionskip}{-0.5cm}
\setlength{\tabcolsep}{3pt}
\scriptsize
% \footnotesize
    \begin{tabular}{l|ccc}
        \toprule[1pt]
         & Training-time & learnable params & total params
        \tabularnewline
        \midrule[1pt]
        FC-CLIP & 30 \textit{h}  & 20.37M & 199.75M\\
        MAFT+ (ours) & 8 \textit{h} & 109.98M & 201.80M \\
        \bottomrule[1pt]
    \end{tabular}
% \vspace{-2mm}
\caption{Params and training times.}
\label{reb-params}
\end{table}
